A Generative Model for Non-Intrusive Load Monitoring in Commercial Buildings

In the recent years, there has been an increasing academic and industrial interest for analyzing the electrical consumption of commercial buildings. Whilst having similarities with the Non Intrusive Load Monitoring (NILM) tasks for residential buildings, the nature of the signals that are collected from large commercial buildings introduces additional difficulties to the NILM research causing existing NILM approaches to fail. On the other hand, the amount of publicly available datasets collected from commercial buildings is very limited, which makes the NILM research even more challenging for this type of large buildings. In this study, we aim at addressing these issues. We first present an extensive statistical analysis of both commercial and residential measurements from public and private datasets and show important differences. Secondly, we develop an algorithm for generating synthetic current waveforms. We then demonstrate using real measurement and quantitative metrics that both our device model and our simulations are realistic and can be used to evaluate NILM algorithms. Finally, to encourage research on commercial buildings we release a synthesized dataset.

==> sections/algo.tex <==
f%!TEX root = ../paper.tex

\section{Semi-Non-Negative Matrix Factorization for NILM}

% \begin{itemize}
% \item Explain why the existing algorithms should fail and motivate the need for a new method
% \item Explain the method
% \end{itemize}

In this section, we review the existing NILM algorithms developed for residential buildings and claim that a method based on semi-non-negative matrix factorization (SNMF) is more suited to the NILM tasks for commercial buildings. 

% developed is based on knowledge acquired on


Since there can be a huge number of similar small devices and several big variable load equipments in commercial buildings, the "one-at-a-time" and the "constant load" hypotheses made by the existing NILM algorithms clearly do not hold. This fact motivates us to consider another type of algorithm from source separation literature. Referred to as matrix factorization, these techniques have been successful in various applications, such as recommendation systems \cite{koren2009matrix} and audio source separation \cite{wang2006investigating}. We have seen that our generative model for current waveforms is based on real signatures and on nonnegative activations. In this context, we propose to apply the semi non-negative matrix factorization (SNMF) algorithm developed by Ding et al \cite{ding2010convex} to the NILM problem.

Let us introduce the SNMF model, with NILM settings \cite{ding2010convex}:
\begin{align}
\min_{S, A}\| I - SA^T \|^2_{\text{Fro}} , \qquad \text{such that } A \geq 0
\end{align}
where $I \in \mathds{R}^{N \times T}$ is the current observation matrix, $S \in \mathds{R}^{N \times C}$ is the signature matrix, $A \in \mathds{R}_{+}^{T\times C}$ is the activation matrix, and $\|M\|_{\text{Fro}}$ denotes the Frobenius norm. Here, each column of $S$ corresponds to a device category and the corresponding column of $A$ will capture the energy consumption of that category. 


In this context, our goal is to estimate the unknown factors $S$ and $A$ after observing the matrix $I$. In \cite{ding2010convex}, the authors develop a gradient-based iterative inference algorithm. Even though their algorithm has nice theoretical convergence properties, in our experiments we have experienced a slow convergence behavior and numerical instabilities. Therefore, for inference we use another alternating optimization schema that can achieve faster convergence rates. 
%
Our approach is based on a coordinate descent schema where at each iteration we solve the problem for only one of the unknown matrices, while keeping the other one fixed. In this case, solving for $S$ while fixing $A$ becomes a least square problem whose exact solution is given as follows:
\begin{align}
S^\star = XA^{\dagger} = XA^T(A^T A)^{-1}.
\end{align}
On the other hand, solving for $A$ while fixing $S$ is a nonnegative least-squares problem that can be solved using Lawson's method \cite{lawson1995solving}.

%  In their paper, Kolter et al \cite{kolter2010energy} use nonnegative matrix factorization (NMF) to disaggregate low frequency power consumption. They start by segmenting the power data on a daily basis and then apply the NMF. They also add a training phase to learn on separate sources (power curve for individual equipment) the signature matrix (composed of daily characteristic power curve).  In our case the observed data is the current and is no longer non negative, this is why we use SNMF.



Although SNMF can be used as an unsupervised learning algorithm, we use it in a supervised setting by learning the factor $S$ from a training dataset, similar to \cite{kolter2010energy}, which uses supervised nonnegative matrix factorization for disaggregating low frequency power consumptions.
%
In the supervised setting, the training phase can be mathematically expressed as follows:
\begin{align}
\min_{\act_c, \sig_c} \|I_c -  \act_c \sig_c^ T\|_{\text{Fro}}^2, \qquad \text{such that } \act_c \geq 0
\end{align}
where $I_c$ contains measurements coming from a single device category, $\sig_c \in \mathds{R}^N$ is a signature vector for category $c$ and $\act_c \in \mathds{R}_{+}^T$ is an activation vector for category $c$. At the end of this training procedure all the estimated $\sig_c$ are concatenated to shape the signature matrix $S = \left[\sig_1, \sig_2, ..., \sig_C\right]$. This learned signature matrix is then fixed during testing and only the matrix $A$ is estimated. 
% used as an initialization for the SNMF task. Note that one can choose to fix the $S$ matrix and not to update it (restraining the problem to a nonnegative least square estimation of $A$). 


==> sections/eval.tex <==
%!TEX root = ../paper.tex

\section{Experimental Validation}
  \label{eval_sec}

\begin{figure}[t]
  \centering
  % \includegraphics[width=0.5\textwidth]{power.png}
  % \includegraphics[width=0.5\textwidth]{synthetic.png}
  \includegraphics[width=0.45\textwidth]{dataset_plots.png}
  \caption{\label{<power>} 1 week samples of residential and commercial buildings total power consumption: public dataset versus synthetic dataset.}
\end{figure}


\subsubsection{Naturalness of the synthetic datasets}
At this point, we also would like to validate that our synthetic datasets share the same characteristics as real datasets. In Figure \ref{<power>}, we can observe that both real and synthesized datasets share the same overall aspect: (a) daily seasonality, continuously varying power for commercial buildings, (b) a peaky power curve and period of constant power for residential ones. Let us look now at the kurtosis of the derivative of the power. Our synthetic commercial dataset has a kurtosis of 5.0 whereas the synthetic residential has a value of 100.5. This values are consistent with the kurtosis observed on the public and private datasets, as shown in Figure \ref{<expkurt>}.

\begin{figure}[]
  \centering
  \includegraphics[width=0.45\textwidth]{simu_kurtosis.png}
  \caption{\label{<expkurt>} Kurtosis of the simulations (used in the experiments), of the two synthetic datasets (released) and the boxplot of real datasets' kurtosis.}
\end{figure}
